LB4OMP: A Dynamic Load Balancing Library for Multithreaded Applications

Exascale computing systems will exhibit high degrees of hierarchical parallelism, with thousands of computing nodes and hundreds of cores per node. Efficiently exploiting hierarchical parallelism is challenging due to load imbalance that arises at multiple levels. OpenMP is the most widely-used standard for expressing and exploiting the ever-increasing node-level parallelism. The scheduling options in OpenMP are insufficient to address the load imbalance that arises during the execution of multithreaded applications. The limited scheduling options in OpenMP hinder research on novel scheduling techniques which require comparison with others from the literature. This work introduces LB4OMP, an open-source dynamic load balancing library that implements successful scheduling algorithms from the literature. LB4OMP is a research infrastructure designed to spur and support present and future scheduling research, for the benefit of multithreaded applications performance. Through an extensive performance analysis campaign, we assess the effectiveness and demystify the performance of all loop scheduling techniques in the library. We show that, for numerous applications-systems pairs, the scheduling techniques in LB4OMP outperform the scheduling options in OpenMP. Node-level load balancing using LB4OMP leads to reduced cross-node load imbalance and to improved MPI+OpenMP applications performance, which is critical for Exascale computing.

==> abstract.tex <==

% Reducing abstract just to better understand the size of the paper

There is a plethora of loop scheduling techniques available in the literature.
The OpenMP standard only specifies three loop scheduling techniques. 
The limited number of scheduling techniques in OpenMP hinders research on novel scheduling techniques since a fair comparison with other existing techniques from the literature is not feasible. 
%A fair comparison with existing techniques from the literature is not feasible for multithreaded applications using \openmp. 
Furthermore, the three scheduling techniques available in OpenMP may not achieve the highest performance for arbitrary applications-systems pairs. 
This work introduces OpenMP library, an extended LLVM OpenMP runtime library that supports fourteen additional \textit{dynamic} loop self-scheduling techniques from the literature. 
%\lbomp offers improved performance for applications and systems in the presence of  unpredictable variations during execution.
%\lbomp is \mbox{open-source} and can easily be used by OpenMP applications with parallel worksharing loops. 
LB4OMP also provides performance measurement features for the analysis of the scheduling and load balancing of OpenMP applications.
We assess the effectiveness of several loop scheduling techniques in multithreaded applications using OpenMP through extensive experimentation. 
We demystify the performance potential and overhead of all standard and newly implemented scheduling techniques in OpenMP using four multithreaded applications executed on three systems.
% The performance analysis shows that for numerous applications-systems combinations, the newly implemented scheduling techniques outperform the standard ones by up to $13.33\%$ (with default chunk size). 
% Extensive experiments with combinations of scheduling techniques for different loops per application-system pair yielded the identification of the highest performing scheduling techniques combination (denoted as \texttt{Best}) for a given application-system pair.
% This work bridges the gap between the state of the art according to the literature and state of the practice of load balancing in multithreaded applications and shows performance improvements that were otherwise unachievable by the \openmp standard scheduling options alone. 
